Abolitionist Networks: Modeling Language Change in Nineteenth-Century Activist Newspapers

The abolitionist movement of the nineteenth-century United States remains among the most significant social and political movements in US history. Abolitionist newspapers played a crucial role in spreading information and shaping public opinion around a range of issues relating to the abolition of slavery. These newspapers also serve as a primary source of information about the movement for scholars today, resulting in powerful new accounts of the movement and its leaders. This paper supplements recent qualitative work on the role of women in abolition's vanguard, as well as the role of the Black press, with a quantitative text modeling approach. Using diachronic word embeddings, we identify which newspapers tended to lead lexical semantic innovations -- the introduction of new usages of specific words -- and which newspapers tended to follow. We then aggregate the evidence across hundreds of changes into a weighted network with the newspapers as nodes; directed edge weights represent the frequency with which each newspaper led the other in the adoption of a lexical semantic change. Analysis of this network reveals pathways of lexical semantic influence, distinguishing leaders from followers, as well as others who stood apart from the semantic changes that swept through this period. More specifically, we find that two newspapers edited by women -- THE PROVINCIAL FREEMAN and THE LILY -- led a large number of semantic changes in our corpus, lending additional credence to the argument that a multiracial coalition of women led the abolitionist movement in terms of both thought and action. It also contributes additional complexity to the scholarship that has sought to tease apart the relation of the abolitionist movement to the women's suffrage movement, and the vexed racial politics that characterized their relation.

==> body-text.tex <==
The Great Work Begins!

The following content is taken from Chang and DeDeo, ``Divergence and the Complexity of Difference in Text and Culture.''

\section{Some figures and citations}

Fig. \ref{fig:operationalization_summary} summarizes our discussion up to this point. We began by distinguishing difference and distance, and pointed out the inherent limitation of distance as embodied experience. Below we shall see divergence in action. It will turn out that divergence, and the underlying epistemic notions it tracks, violates the axioms of distance---``symmetry'' and ``no shortcut'' in particular---in crucial and useful ways.

\begin{figure}[H]%[!htbp]
  \centering
  \includegraphics[width=0.75\textwidth]{fig/summary.pdf}
  \caption{Two paths to operationalizing difference: a cognitive approach made possible by the information-theoretic notion of divergence provides a different account of how things differ than the more familiar spatial metaphor of distance.}
  \label{fig:operationalization_summary}
\end{figure}

Given an interpretive frame, we can often consider one text as being broader, or ranging over more themes, than another. One can then speak of the asymmetrical relationship of one text being contained, or enclosed, by another. Consider, for example, the case of diction. At any particular time, a culture will have a range of registers available for a text to use~\autocite{bachtin2011Dialogic}. One text may have an elevated diction, another low, and a third might mix the two. A recent study by Stefania Degaetano-Ortlieb and Elke Teich shows how scientific English became broader, or gradually came to \textit{enclose}, general English over the second half of the nineteenth century.\footnote{See~\fullcite{degaetanoOrtlieb2019Optimal}, where they establish this ``subtle effect'' of scientific language enclosing general English in passing. They do so precisely in the way we argue for here, by reference the asymmetric nature of KL divergence. In their phrase, which captures the cognitive aspect of the information theoretic quantities in play, the enclosure relationship indicated by the KL asymmetry implies that general English is a worse ``model'' for scientific English than vice versa. See also~\fullcite{DegaetanoOrtlieb2019b}.} There are certainly words that are common in general English that are less common in scientific English (for example, the word ``wife''). However, there are (roughly speaking) far more words in scientific English that are rarely, if ever, used in general English (such as ``oxide''). This imbalance is measured by the Kullback--Leibler asymmetry.

\section{Some tables}

To drive this intuition, consider two major words of Russian literature, \emph{Anna Karenina} and \emph{War and Peace}, by Leo Tolstoy. In a very general sense (and the only one needed to understand this example), both of these novels deal with themes of friendship, suffering, war, and love, but in different proportions; while \emph{Anna Karenina} is most famously centered around a love story, \emph{War and Peace} follows a variety of characters as they navigate a broader array of life events.

We can represent, in this toy example, the two novels as probability distributions over these themes. Explicitly, the distributions $p_A$ (\emph{Anna Karenina}) and $p_B$ (\emph{War and Peace}) quantify the themes by reference to the relative proportions of words associated with the core concepts in order, as in table~\ref{tab:novelthemes}:\footnote{For this toy example, friendship words are: friend, friendship, companionship, fellowship, camaraderie; suffering words are: suffering, hurt, ache, pain, agony, miserable, wretched; war words are: war, conflict, warfare, combat, fighting, struggle, armed, military, bloodshed; and love words are: love, lover, fondness, tenderness, warmth, intimacy, attachment, endearment.}
\begin{eqnarray*}
p_A & =  & \{0.14, 0.21, 0.08, 0.57\}, \\
p_B & =  & \{0.15, 0.15, 0.37, 0.36 \}.
\end{eqnarray*}
Intuitively, at this level of analysis, \emph{War and Peace} covers a broader range of themes than \emph{Anna Karenina}; the latter, for example, distributes only 8\% of its coverage to war, compared to 37\% in \emph{War and Peace}.

\begin{table}[H]%[!htbp]
  \fontsize{12}{12}\selectfont
  \centering
  \begin{tabular}{@{}llll@{}}
    \toprule
    theme      & \emph{Anna Karenina} & \emph{War and Peace} \\
    \midrule
    friendship & 14\%    & 15\% \\
    suffering  & 21\%    & 12\% \\
    war        & 8\%     & 37\% \\
    love       & 57\%    & 36\% \\
    \bottomrule
  \end{tabular}
  \caption{While \emph{Anna Karenina} is dominated by words associated with love, \emph{War and Peace} has a more uniform distribution over the four themes considered here. In this sense, \emph{War and Peace} ``encloses'' the themes in \emph{Anna Karenina}, and while the Kullback--Leibler from \emph{Anna Karenina} to \emph{War and Peace} is 0.49 bits, the Kullback--Leibler in the reverse direction, from \emph{War and Peace} to \emph{Anna Karenina}, is only 0.35 bits. In this example, the compositions of the two novels are determined by counting words associated with the four themes in the English-language translations of Constance Garnett and computing the relative odds. The listed probabilities are then conditional probabilities: given that one has encountered one of these themes, what are the probabilities that it was this one or that.}\label{tab:novelthemes}
\end{table}


The Kullback--Leibler Divergence reflects these differences in the asymmetry between the two directions. The KL from \emph{Anna Karenina} to \emph{War and Peace} (i.e., ``the surprise on reading \emph{Anna Karenina} and then encountering \emph{War and Peace}, when one searches for these themes''), is $0.49$ bits, while the KL from \emph{War and Peace} to \emph{Anna Karenina} is $0.35$ bits. The enclosure relationship is captured in the asymmetry, or difference, in surprise.\footnote{Formally, our operationalization of enclosure, $\textrm{KL}(p_1|p_2)-\textrm{KL}(p_B|p_A) > 0$, indicates that $p_A$ encloses $p_B$.} In this interpretative framework, readers who begin with \emph{Anna Karenina} have little exposure to narratives involving war; when they read \emph{War and Peace}, they encounter new patterns associated with the war theme more than one third of the time. Conversely, readers who begin with \emph{War and Peace} have significant exposure to all four themes; they see less representation of some of them than they would in \emph{Anna Karenina}, but not enough to overcome the near-total absence of war in the latter. The underlying asymmetry of $0.074$ bits between the texts, in the direction from \emph{War and Peace} to \emph{Anna Karenina}, captures this relationship.


==> ca-sty/articleinfo.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% EDITOR'S ZONE
\newcommand{\pubdate}{\today}

% this appears right after the author names
\newcommand{\articleinfocontent}{%
Peer-Reviewers:David Smith, Richard Jean So\\
Dataverse DOI:10.7910/DVN/EWYMFG
}

% first-page footer
\fancypagestyle{plain}{%
  \renewcommand{\headrulewidth}{0pt}%
  \fancyhf{}%
  \fancyfoot[C]{\small%
  \textit{Journal of Cultural Analytics} 1 (2021): 1-43. doi: 10.22148/001c.18841%
  }%
}

==> ca-sty/ca-sty.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FONT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{anyfontsize}
\usepackage[no-math]{fontspec}
\usepackage{mathspec}
\defaultfontfeatures{Mapping=tex-text}

\setmainfont{Times New Roman}[%
  Path            = ca-sty/fonts/,%
  Extension       = {.ttf},%
  UprightFont     = {*},%
  BoldFont        = {* Bold},%
  ItalicFont      = {* Italic},%
  BoldItalicFont  = {* Bold Italic}]

\setsansfont{Arial}[%
  Path            = ca-sty/fonts/,%
  Extension       = {.ttf},%
  UprightFont     = {*},%
  BoldFont        = {* Bold},%
  ItalicFont      = {* Italic},%
  BoldItalicFont  = {* Bold Italic}]

\setmathsfont(Digits,Latin)[%
  Path            = ca-sty/fonts/,%
  Extension       = {.ttf},%
  UprightFont     = {*},%
  BoldFont        = {* Bold},%
  ItalicFont      = {* Italic},%
  BoldItalicFont  = {* Bold Italic}%
]{Times New Roman}

\setmathrm[%
  Path            = ca-sty/fonts/,%
  Extension       = {.ttf},%
  UprightFont     = {*},%
  BoldFont        = {* Bold},%
  ItalicFont      = {* Italic},%
  BoldItalicFont  = {* Bold Italic}%
]{Times New Roman}

\newfontfamily\relaxed[%
  WordSpace=1.8,%
  LetterSpace=14,%
  Path            = ca-sty/fonts/,%
  Extension       = {.ttf},%
  UprightFont     = {*},%
  BoldFont        = {* Bold},%
  ItalicFont      = {* Italic},%
  BoldItalicFont  = {* Bold Italic}%
]{Times New Roman}

% \usepackage{mathptmx}
% \usepackage{helvet}
% \usepackage[letterspace=200,tracking=true]{microtype}
% \let\relaxed\lsstyle

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LAYOUT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[%
  a4paper,%
  hmargin = 1in,
  includehead,
  headheight = 1in,
  footskip = 0.5in,
  tmargin = 0mm,
  bmargin = \dimexpr1.5in+\ht\strutbox\relax,
   footnotesep = 0.5in plus 4pt minus 4pt
]{geometry}
\setlength{\parskip}{12pt}
\setlength{\parindent}{0pt}
\renewcommand{\baselinestretch}{1.15}
\usepackage[document]{ragged2e}


% color
\usepackage{xcolor}
\definecolor{ca}{RGB}{59,79,141}

% caption
\usepackage{float}
\usepackage{caption}
\DeclareCaptionFormat{ca}{\itshape\fontsize{10}{11}\selectfont#1#2#3}
\captionsetup{format=ca}

\usepackage{hyperref}
\usepackage{tikz}
\usepackage{adjustbox}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FOOTNOTE/ENDNOTE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Chicago style
\usepackage[notes,backend=biber,%
  includeall=false,booklongxref=false,%
  compresspages,noibid,doi=only,autolang=other,%
  bibencoding=inputenc,footmarkoff%
]{biblatex-chicago}
\newcommand\mfs{\textsuperscript{,}\nobreak}
% Those two packages clash but it doesn't really matter much
%\addtolength{\skip\footins}{2pc plus 5pt}
\usepackage{footmisc}
\usepackage{endnotes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Header and footer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{fancyhdr}
\fancyhf{}
\renewcommand{\footrulewidth}{0pt}
\fancyhead[CE]{\fontsize{8}{10}\selectfont\MakeUppercase{\relaxed \headertitle}}
\fancyhead[CO]{\fontsize{8}{10}\selectfont\MakeUppercase{\relaxed Journal of Cultural Analytics}}
\fancyfoot[C]{\thepage}
\pagestyle{fancy}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DON'T TOUCH THIS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}
\renewcommand{\maketitle}{\bgroup
  \renewcommand{\footnoterule}{}
  \renewcommand\@makefnmark{}
  %%
  \renewcommand\@makefntext[1]{%
    \parindent 0pt%
    \sffamily\fontsize{8}{12}\selectfont%
    {}
  ##1}
 %%
  \newcommand\authorinfo[1]{%
    \begingroup
      \renewcommand\thefootnote{}\footnote{##1}%
      \addtocounter{footnote}{-1}%
    \endgroup 
  }
 \begin{minipage}[t]{\textwidth}
   \vspace*{-1in}
   \begin{tikzpicture}
     \node[inner sep=0] (header) at (0,0){\includegraphics[width=\textwidth]{ca-sty/ca-header.pdf}};
     \node[left,text width=4.4cm,align=center,yshift=-3pt] at (header.east){\color{ca}\sffamily\fontsize{12}{12}\selectfont\pubdate};
  \end{tikzpicture}
  %%
  \vspace{16pt}\\ % 14 + 16 = 30 (= 6+24)?
  %%
  {\sffamily\bfseries\fontsize{24}{24}\selectfont\@title\par}
  \vspace{6pt}
  {\color{ca}\sffamily\fontsize{12}{12}\selectfont\@author\par}
\end{minipage}
\egroup
%\bigskip
}

\renewenvironment{abstract}{%
  %\vspace{6pt}
  {\sffamily\fontsize{8}{12}\selectfont\articleinfocontent\par}
  \begin{adjustbox}{minipage=0.8\textwidth,center}
   \vspace{12pt}
    {\centering\noindent\fontsize{9}{9}\selectfont%
      \MakeUppercase{\bfseries\relaxed Abstract}\par}
    \vspace{-0.5\baselineskip}
    \noindent\rule[2pt]{\columnwidth}{0.5pt}\\
    \fontsize{7.5}{7.5}\selectfont%
    %\justify
}{%
 \par
 \noindent\rule{\textwidth}{0.5pt}
 \end{adjustbox}
 \vspace{12pt}
 %\vspace{-\bigskipamount}
}
\makeatother

\usepackage[explicit]{titlesec}
\titleformat{\section}%
  {\fontsize{18}{18}\selectfont\bfseries}{}{0pt}{#1}
% \titlespacing{command}{left spacing}{before spacing}{after spacing}[right]
\titlespacing{\section}{0pt}{12pt}{6pt}

\titleformat{\subsection}%
  {\fontsize{16}{16}\selectfont\itshape}{}{0pt}{#1}
\titlespacing{\subsection}{0pt}{6pt}{3pt}

\titleformat{\subsubsection}%
  {\fontsize{14}{14}\selectfont\bfseries}{}{0pt}{#1}
\titlespacing{\subsubsection}{0pt}{3pt}{3pt}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> src/050experiments.tex <==
%%TC:ignore
\section{Experimental Setup}
\label{sec:experiments}

\todo{Moved all this content back up to the "data setup" section of the Data section, above. Check to see that it's OK and then delete this section.}
\paragraph{Data setup} We divide the corpus into 10 equal timespan intervals. We also group \newspaper{Douglass Monthly}, \newspaper{Frederick Douglass Paper} and \newspaper{The North Star} into a single source \newspaper{Douglass Papers}. Similarly, \newspaper{The Colored American} and the \newspaper{The Weekly Advocate} is grouped into \newspaper{The Colored American}. Newspapers that do not contain at least 500 articles throughout their tenure in the period of interest are ignored. \todo{say how many newspapers remain}  

\paragraph{Model setup} Words that appear less than 5 times throughout the corpus are not included in the vocabulary. Moreover, the vocabulary is limited to the 50K most frequent words in the corpus. The embedding size for all the models is set to 100 dimensions. The window size to determine the context words is set to 5 in both directions. The parameters of all the models are L2-regularized with the coefficient set to $10^{-4}$.

\todo{maybe also the right place to mention the word filters to remove false flag changes after the temporal models.}
%%TC:endignore
